TutteNet: Injective 3D Deformations by Composition of 2D Mesh Deformations

This work proposes a novel representation of injective deformations of 3D space, which overcomes existing limitations of injective methods: inaccuracy, lack of robustness, and incompatibility with general learning and optimization frameworks. The core idea is to reduce the problem to a deep composition of multiple 2D mesh-based piecewise-linear maps. Namely, we build differentiable layers that produce mesh deformations through Tutte's embedding (guaranteed to be injective in 2D), and compose these layers over different planes to create complex 3D injective deformations of the 3D volume. We show our method provides the ability to efficiently and accurately optimize and learn complex deformations, outperforming other injective approaches. As a main application, we produce complex and artifact-free NeRF and SDF deformations.

==> bakup/0_abstract.tex <==
\begin{abstract}
\vspace{-0.1in} %%%%%%
This work proposes a novel representation of injective deformations of 3D space, which overcomes existing limitations of injective methods, namely inaccuracy, lack of robustness, and incompatibility with general learning and optimization frameworks. Our core idea is to reduce the problem to a ``deep'' composition of multiple 2D mesh-based piecewise-linear maps.  Namely, we build differentiable layers that produce mesh deformations through Tutte's embedding (guaranteed to be injective in 2D), and compose these layers over different planes to create complex 3D injective deformations of the 3D volume. We show our method provides the ability to efficiently and accurately optimize and learn complex deformations, outperforming other injective approaches. As a main application, we  produce complex and artifact-free NeRF and SDF deformations.
\end{abstract}

==> bakup/1_intro.tex <==
\vspace{-15pt}
\section{Introduction}
\label{sec:intro}
% \vspace{-0.05in}
%what is it about
This work concerns computation and learning of 3D deformations.
%why important
As the most immediate mode of manipulation and interaction with 3D shapes, deformations play a crucial role in various fields such as vision~\cite{wang2023tracking}, medical imaging~\cite{lv2022joint}, 3D registration~\cite{deng2022survey},  and graphics~\cite{skinningcourse:2014}. 
%injectivity is important
In many real-world applications, it is crucial that the deformation does not create any self-overlaps, i.e., is \emph{injective} (a 1-to-1 mapping). An example that is a key motivation for this work, is deformation of  Neural Radiance Fields (NeRFs)~\cite{nerf}: when deforming NeRFs, lack of injectivity can easily cause severe rendering artifacts due to intersecting ``deformed'' rays during the ray tracing process, see Figure~\ref{Figure:nerf_cage}. 

% \vspace{-0.03in}
Unfortunately, current approaches do not provide an injective deformation method that is both sufficiently expressive and robust, as well as lending itself to practical optimization and learning: 
%geometry processing mesh

-- On one hand, within geometry processing and graphics,  3D deformations are heavily-researched through triangular/tetrahedral \emph{mesh} deformations, i.e., modifying the position of each vertex of the mesh. Mesh deformations provide a finite set of meaningful geometric degrees of freedom leading to stable, quick,  and straightforward computation, as well as access to geometric quantities such as the deformation gradients (\textit{Jacobians}), critical in most mesh-deformation approaches~\cite{xu2009gradient}. However, mesh deformations cannot be \emph{learned} while ensuring injectivity, nor are directly applicable when an explicit triangulation of the shape is not given. 
%learning methods

-- On the other hand, the ML community has heavily-researched \emph{functional} representations of injective maps via neural networks, such as normalizing flows~\cite{realnvp} and solutions to ODEs~\cite{chen2018neural}. These methods were mainly designed for high-dimensional mappings, e.g., for generative tasks~\cite{grathwohl2018ffjord}, but have recently been successfully adapted to injective 3D deformations~\cite{wang2023tracking,huang2020meshode,jiang2020shapeflow}. The functional representation which they provide is not geometric, but rather embedded abstractly within the network's weights, resulting in many cases in slow, cumbersome and unstable computation, possibly leading to a less-accurate prediction, or practical intangibility of critical geometric quantities such as the aforementioned deformation Jacobians. 

% \noam{talk about not wanting to mesh}
In this work, we aim to resolve these issues and gain the benefits of both worlds: we propose a novel computational representation for 3D injective deformations, which \textit{combines} the geometric representation of mesh-based deformations with the standard deep-learning approach of functional composition. 

Our core observation is that sequentially composing multiple 2D mesh deformations, over different 3D planes, achieves two critical goals simultaneously: 1) similarly to other ``deep'' representations, compositionality leads to an expressive representation, able to capture complex 3D deformations accurately, while simultaneously using mesh deformations for its layers, providing virtues such as numerical stability and accuracy; 2) while injectivity is not directly tractable for 3D mesh deformations, it is in 2D. Hence, by reducing each deformation ``layer'' to 2D, we can leverage recent observations for 2D injective mesh deformations~\cite{escher}, which show how 2D Tutte embeddings~\cite{tutte1963draw} can yield a differentiable parameterization of \emph{all} injective mesh deformations into a convex domain, enabling unconstrained learning and  optimization. Composing multiple 2D injective deformations from different viewpoint defines a family of injective volumetric 3D deformations. 
% \noam{we avoid explicit triangulation emphasize}
% \noam{reference table: Through this representation}
% which is tailored for their learning and optimization. Namely, it holds three key properties necessary for practical use within learning and optimization pipelines:  1) \textbf{Expressiveness.} it is highly expressive, and can accurately capture and represent complex deformations; 2) \textbf{Injectivity.} It is guaranteed to produce injective maps by construction, thereby removing the need to, e.g., regularize the output to be injective; 3) \textbf{Parameterized}\noam{better name for this property?}it lends itself easily to optimization and learning, by exposing a set of parameters that directly control the injective deformation.


% \noam{our core observation is that the space of 3D PL mappings is tractable thorugh a compisition of 2D PL maps, as there exist methods to ensure 2D PL maps are injective.}
% Our core idea for devising this expressive space of 3D injective deformations is to build a ``deep'' model of 3D piecewise-linear (PL) maps. PL maps are ubiquitous in geometry processing, graphics, physics simulation, and engineering, due to their high expressiveness and ability to approximate arbitrary maps.  However, there is no tractable representation for \emph{injective} 3D PL maps.  Instead, we concatenate multiple 2D planar PL deformation ``layers'' over different planes, thereby reducing the problem to designing a 2D injective deformation layer, which is tractable: we triangulate the 2D domain (a square) and optimize over the space of all injective 2D piecewise-linear deformations of that triangulation, by controlling Tutte embeddings~\cite{tutte,floater,escher}. 
% This space of injective maps is highly expressive, and is guaranteed to well approximate any given injective deformation, for a fine enough triangulation. 
% Through concatenation of these planar maps, the resulting 3D deformation is injective, directly controllable, and expressive.


% sequentially apply a series of piecewise-linear (PL) deformations. 
% sFollowing the ``deep'' paradigm, we stack multiple layers of deformations on one another, each acting on the output of the previous layer, providing greater expressivness than possible with a single layer.  use 
% PL mappings are ubiquitous in geometry processing, graphics, physics simulation, and engineering, as a highly-expressive deformation model. However, there is no tractable representation of 3D inejctive deformations. Concatenating multiple PL deformations on top of one another thus achieves two goals simultaneously: first, similarly to the layers of a \emph{deep} neural network, by sequentially applying additional deformation ``layers''


% Since there  we instead 


\begin{table}[t]
\centering
\setlength{\tabcolsep}{2.5pt}
\scalebox{0.82}{
\begin{tabular}{lccccc cccc}
\toprule  
& \multirow{2}{*}{Learnable} & \multirow{2}{*}{\makecell[b]{Analytical \\ inverse}} & \multirow{2}{*}{\makecell[b]{Fast Det. \\ Jacobian}}  & \multirow{2}{*}{\makecell[b]{Fast full \\ Jacobian}}  & \multirow{2}{*}{\makecell[b]{Robustness}}\\
\\
\midrule  %

i-ResNet~\cite{iresnet} & $\greencheckmark$ &  $\redxmark$ &  $\redxmark$  &  $\redxmark$ & $\redxmark$ \\ 
RealNVP~\cite{realnvp} & $\greencheckmark$ &  $\greencheckmark$ & $\greencheckmark$ & $\redxmark$ & $\redxmark$ \\
NeuralODE~\cite{chen2018neural} & $\greencheckmark$ & $\greencheckmark$ &  $\greencheckmark$ &  $\greencheckmark$  & $\redxmark$\\
\midrule  %

Ours & $\greencheckmark$  & $\greencheckmark$ & $\greencheckmark$ & $\greencheckmark$ & $\greencheckmark$ \\
\bottomrule
\end{tabular}
}
\caption{{\bf Properties of injective deformation methods.} Beyond superiority in accuracy and efficiency, our method holds unique properties compared to other injective methods, see Sec.~\ref{section:method:properties}.}
\label{tab:properties}
\vspace{-15pt} %%%% \vspace{-20pt 
\end{table}
We show through experiments that our method can be used both for accurately \textit{learning} injective deformations (e.g., learning to repose a given human model to arbitrary poses), as well as \textit{optimizing} volumetric deformations in tasks in which injectivity is critical, e.g., elastically deforming a NeRF with respect to user interactions. Through comparisons, we show that our method significantly outperforms other injective deformation techniques. Furthermore, through comparisons to previous (non-injective) NeRF-deformation techniques, we both exhibit the importance of injectivity, as well as show that in many cases our method is still more expressive than those competing techniques, in spite of them facing a less-constrained problem. %\thibaultrmk{Mention word ``TutteNet'' somewhere}
% \begin{table}
% \setlength\extrarowheight{2pt}
% \centering
% \caption{Injective deformation methods.}\label{Tab1}
% \begin{tabular}{p{0.15\columnwidth}|p{0.15\columnwidth} | p{0.15\columnwidth} | p{0.15\columnwidth} | p{0.15\columnwidth}}
% \hline
%  & \textbf{Learnable} & \textbf{Analytical Inverse}
%     & \textbf{Fast Jacobian Access} & \textbf{Explicit Map}  \\ 
% \hline
% &\tabyes & \tabno & \tabyes & \tabno 
% \end{tabular}
% \label{tab:properties}
% \end{table}


% \noam{previous:}
% Antoine Lavoisier, a renowned 18th century french chemist famously said ``Nothing is lost, nothing is created, everything is transformed.'' The same principle holds true in 3D mesh deformation. A 3D deformation method, whether it operates on surface meshes, or volumes like NeRFs, should never collapse 3D content nor make it disappear. \noam{check this out}Mathematically, the notion is called injectivity : two points in the input domain of a function have different outputs. 

% Creating 3D injective maps have been a long-standind challenge in 3D deformation because the space of 3D bijection have proven very hard to parameterize. 
% On the other hand, with one less dimension, one can caracterize the space of 2D bijection over a domain with fixed boundaries using the well-known Tutte embeddings~\cite{}. Unfortunatly, it is well known that these transformation do not extend easily to 3D.
% To address this concern, we propose to parameterize a familly of 3D bijection by composing multiple 2D Tutte deformation layers via orthographic projection to different planes. The resulting deformation space is highly expressive and well suited to perform machine learning.

% We demonstrate ...

% In summary, our main contributions is a novel parameterizion of 3D bijective mappings via composition of 2D Tutte layers.



==> bakup/2_related_work.tex <==




\section{Related Work}
\label{sec:related_work}

\paragraph{Invertible neural networks.} Injective maps are critical for generative modeling, in order to map between distributions. This has fueled the development of families of invertible neural functions. Normalizing Flows~\cite{dinh2014nice, germain2015made, salimans2015markov, maf, iaf, oord2016wavenet, realnvp, rezende2015variational, trippe2018conditional} are highly prominent, with RealNVP~\cite{realnvp} applied to 3D volume deformations, e.g., long-range optical flow~\cite{wang2023tracking} or for learning 3D deformations~\cite{Lei2022CaDeX,Paschalidou2021CVPR}. They work by defining an injective transformation of a subset of the spatial coordinates at each block, which is ideal for a high-dimensional settings but loses expressivity when the subsets must lie in 1D/2D. Continuous flows through Neural solutions to Ordinary Differential Equation (NeuralODE)~\cite{chen2018neural} have also been successfully applied to 3D deformations, e.g., for shape autoencoding~\cite{gupta2020neural}, dynamic mesh reconstruction~\cite{OccupancyFlow},  for point cloud generation~\cite{yang2019pointflow} and  asset deformation~\cite{huang2020meshode, jiang2020shapeflow}. Finally, i-ResNet~\cite{iresnet} achieves invertibility of a ResNet by enforcing Lipschitz bounds, with~\cite{yang2021geometryprocessingneuralfields} using this formulation for 3D deformations. We empirically evaluate and compare to these methods in Section~\ref{sec:exp:learn}. In Table~\ref{tab:properties}, we compare desirable properties for 3D invertible deformations.  \our{} can be considered as a variant of a normalizing flow, however is an explicit representation through composition of geometrically-expressive 2D mesh deformations, designed specifically for geometric 3D deformations, without the inclusion of a neural network in the deformation process.




% Paschalidou2021CVPR : to discover semantically meaningfull parts in 3D object collections
% Lei2022CaDeX : 
 % We need the explicit Jacobian of the transformation (not just its determinant) to optimize typical 3D deformation energies~\cite{arap}, which is very slow to compute for RealVPN, as it does with autodiff. In contrast, we have an analytical formulation of the determinant yielding 1000x faster inference time. + empirical evidence of expressivity.
\vspace{-4mm} %%%%%% \vspace{-3mm}
\paragraph{Injective deformations of meshes in geometry processing.} 
\begin{figure*}[t]
\centering
% \begin{overpic}[width=1\textwidth]
\includegraphics[width=1\textwidth]{Figures/tuttenet_diagram2.pdf}
% \end{overpic}
\caption{\textbf{Our representation of injective 3D deformations}, visualized for the process of mapping a given point $\p$ inside the volume, for two-layer \our{}, $i\in\set{1,2}$. Left: the (learnable) parameters $\theta^i$, consisting of the mesh-Laplacian $\lap^i$ and the boundary conditions $\bdry^i$, define a 2D deformation $\planlayer^i$ of the square mesh $\mesh$, through Tutte's embedding~\cite{tutte1963draw}. $\planlayer^i$ is embedded in 3D to the local coordinates $\rotation^i$ to define a 3D deformation, $\layer^i$. Right: given a point $\p$, it is projected to the local coordinates of $\layer^1$, landing on triangle $\tri^1$.  $\layer^1$  defines an affine map over the infinite prism of $\tri^1$ (represented in blue with dotted lines), mapping $\p$ to $\layer^1(\p)$. The resulting $\layer^1\parr{\p}$ is projected onto the local coordinates of $\planlayer^2$, landing on triangle $\tri^2$, from which it is mapped by the affine map $\layer^2$ defined over the infinite prism of $\tri^2$.   }
\label{fig:diagram}
\vspace{-0.0in}
\end{figure*}
3D injective deformations have been extensively researched in geometry processing, mainly for piecewise linear maps on triangle meshes. Local and global injectivity can be achieved through energies that encourage or enforce it~\cite{schuller2013locally,smith2015bijective, slim,du2021optimizing,garanzha2021foldover} but cannot guarantee injectivity when additional objectives are added, or in learning settings. Injectivity can be achieved via convex constraints~\cite{aigerman2013,kovalsky2014controlling}, tailor-made solvers~\cite{li2020incremental}, or discrete modifications of the triangulation to preserve or recover injectivity~\cite{simplexassembly,jiang2017simplicial,muller2015air} that cannot be applied in a learning setting or without a well-defined triangle mesh. Other methods use non-discrete representations~\cite{campen2016bijective} that cannot be predicted or optimized. We use layers of 2D injective deformations define via Tutte's embedding~\cite{tutte1963draw,floater2003one}, and control each  layer by the method proposed in~\cite{escher}, of optimizing the mesh Laplacian and boundary conditions. 

\vspace{-0.12in} %%%%%%% 
\paragraph{NeRF Deformation.}
% \noam{add SDF deformation  also to conclusion}
Several works use 3D volume deformations defined by MLPs that input/output spatial coordinates as a means to achieve various applications for NeRF, e.g.,  dynamic scenes~\cite{gao2021dynamicview, wu20234dgaussians, park2021hypernerf,park2021nerfies, tretschk2021nonrigid}, stylization~\cite{xu2023desrf}, and controlling trajectories~\cite{editingnerf}. Other works focus on providing NeRF deformation tools for end users, usually via a proxy geometry that controls the volume deformation, e.g., using a mesh scaffold and transfers a user-defined mesh deformation to a volume deformation Nerf-Editing~\cite{nerfediting},  or through enveloping cages~\cite{cagenerf, deformingRFCages, NeRFshop23cage, li2023interactivecage}. Others \emph{bake} the NeRFs  into a more deformation-friendly representation, such as meshes~\cite{neumesh} or point clouds ~\cite{liang2022spidr,neuraleditor}.
None of these approaches is injective nor can be applied to a NeRF without a preprocessing step of fitting the proxy to the NeRF, making learning and optimization less straightforward. We compare with \cite{nerfediting, deformingRFCages, liang2022spidr} and demonstrate the importance of injectivity. Many other learning techniques exist for deforming shapes that are not NeRFs, e.g., by predicting per-points offsets via coordinate-based MLPs~\cite{atlasnet, 3DCODED, yang2018foldingnet, fan2017pointsetgen, tancik2021learned, Park_2019_CVPR, chen2019learning,mescheder2019occupancy, deng2021deformed},  Jacobians~\cite{aigerman2022neural},  rigs~\cite{holden, li2021learning, AnimSkelVolNet, RigNet, neuroskinning,neuralcages}, or point handles~\cite{jakab2021keypointdeformer,liu2021deepmetahandles}. To avoid self-intersection, they often rely on regularizing the Jacobian~\cite{bednarik2020shape,arap, huang2021arapreg} or the Laplacian~\cite{kanazawa2018learning}.



% \paragraph{Learning 3D deformation}
% Neural Jacobian Fields~\cite{aigerman2022neural}





==> bakup/3_method.tex <==
% \begin{figure*}[t]
% \centering
% % \begin{overpic}[width=1\textwidth]
% \includegraphics[width=1\textwidth]{Figures/tuttenet_diagram.pdf}
% % \end{overpic}
% \caption{\textbf{Our representation of injective 3D deformations}, visualized for the process of mapping a given point $\p$ inside the volume, for two-layer \our{}, $i\in\set{1,2}$. Left: the (learnable) parameters $\theta^i$, consisting of the mesh-Laplacian $\lap^i$ and the boundary conditions $\bdry^i$, define a 2D deformation $\planlayer^i$ of the square mesh $\mesh$, through Tutte's embedding~\cite{tutte1963draw}. $\planlayer^i$ is embedded in 3D to the local coordinates $\rotation^i$ to define a 3D deformation, $\layer^i$. Right: given a point $\p$, it is projected to the 3D embedding of $\planlayer^1$, landing on triangle $\tri^1$.  $\layer^1$  defines an affine map over the infinite prism of $\tri^1$ (represented in blue with dotted lines), that maps $\p$ to $\layer^1(\p)$. The resulting $\layer^1\parr{\p}$ is then projected onto the 3D embedding of $\planlayer^2$, landing on triangle $\tri^2$, from which it is mapped by the affine map $\layer^2$ defines over the infinite prism of $\tri^2$.   }
% \label{fig:diagram}
% \vspace{-0.2in}
% \end{figure*}

\section{Method}
\label{method}
We now describe our expressive representation of 3D injective functions through composition of 2D injective mesh deformations, see Figure~\ref{fig:diagram} for visualization of the full pipeline. We begin by setting some necessary preliminaries regarding piecewise-linear maps and Tutte embeddings (Section~\ref{section:method:pre}), then describe our representation (\ref{section:method:representation}) and conclude with analyzing its core properties (\ref{section:method:properties}).

 \subsection{Preliminaries} 
 \label{section:method:pre}
 \paragraph{Piecewise-linear maps.} We assume to have a 2D triangular mesh $\mesh$ with triangles $\T$ and vertices $\V$ embedded in $\rtwo$. $\mesh$ can be any disk-topology mesh - in all experiments, we use the unit square, $\Omega=\brac{-1,1}^2$, and triangulate it with a regular triangulation of same-size isosceles triangles. We consider 2D piecewise-linear maps $\planlayer:\mesh\to\rtwo$ of this mesh, meaning the map is affine over each triangle $\tri\in\T$,  
 \begin{equation}
 \label{eq:2jac}
     \planlayer\vert_\tri\parr{\p} \equiv A_\tri \p+\delta_\tri, 
 \end{equation}
 for some $A_\tri\in\mats{2}{2},\delta_\tri\in\real^2$. (Note that this map can map \emph{any} point $\p\in\Omega$ and not just the vertices of a mesh).  The gradient of a map at point $\p$, denoted $D_\p\Psi$, is called the \emph{Jacobian}. For piecewise-linear maps, the Jacobian is constant over each triangle $\tri$ and is exactly the linear transformation $D_\tri\Psi=A_\tri$. To define a continuous piecewise linear map $\planlayer$, it suffices to define deformed vertex positions $\U=\set{\uertex_i}_{i=0}^{\abs{\V}}$, assigning position $\uertex_i\in\rtwo$ to each vertex $\vertex_i\in\V$, and define the map via $\planlayer\parr{\vertex_i} = \uertex_i$.
 Given $\uertex_i$ the Jacobian can be obtained by solving the linear equation \begin{equation}
 \label{eq:map_from_vert}
     A_\tri \vertex_i  + \delta_\tri= \uertex_i,\ i\in\tri
 \end{equation} w.r.t $A_\tri$ - the resulting small $6\times6$ linear equations can be inverted \emph{once} at initialization of training/optimization. 



 
 

\paragraph{Tutte's embedding} is a method for computing injective 2D mesh mappings~\cite{tutte1963draw,floater2003one}, for meshes with disk topology (i.e., having one loop of boundary vertices). Given a mesh-Laplacian matrix $\lap$, defined by assigning some positive scalar $\lap_{ij}\in\real^+$ to each edge $\parr{i,j}$ of the mesh $\mesh$, along with a sequence of 2D points $\bdry_1,...,\bdry_k\in\rtwo$ that lie on a convex polygon, Tutte's embedding computes  deformed vertex positions $\U = \set{\uertex_i}_{i=0}^{\abs{\V}}$ by solving the sparse linear system defined via:
\begin{equation}
\label{eq:tutte}
\begin{split}
    \sum_{j}\lap_{ij}&\parr{\uertex_j-\uertex_i} = 0  \text{ for each interior vertex $\vertex_i$}\\
    &\uertex_i = \bdry_i  \text{ for each boundary vertex $\vertex_i$. }
\end{split}
\end{equation}
While Tutte's embedding is guaranteed to be injective in 2D, it is unfortunately well-known to not hold in 3D (see, e.g., ~\cite{campen2016bijective}) hence extensions to 3D do not exist. 

\subsection{3D injections through 2D mesh deformations} 
\label{section:method:representation}
% We are looking for a way to learn and optimize injective functions  $\map_\theta: \bij{\rthree}{\rthree}$\noam{need to mention somewhere it's actually something like the unit ball}, that is parameterized by some set of parameters $\theta$. We further aim to have these functions be piecewise-linear maps, as these guarantee good properties and expressive capabilities. Unfortunately, there is no method to provide a tractable representation of a space of injective piecewise-linear maps in 3D. Thus, instead, our approach is to reduce the 3D injective piecewise-linear mapping problem to a sequence of 2D piecewise-linear injective mapping problems. 
We wish to devise an optimizable family of injective deformations $\map_\theta$ of 3D volumetric space, which leverages mesh deformations. Since no simple parameterization of injective 3D mesh deformations is known, the key idea of TutteNet is instead to define the 3D deformation through the composition of 2D injective mesh deformations (see Figure~\ref{fig:diagram}).

\vspace{-0.1in} %%%%%% 
\paragraph{Prismatic layers.}Postponing the discussion on how to compute 2D injective mesh deformations, assume for now that we have one such injective 2D mesh deformation, ${\planlayer:\bij{\mesh}{\rtwo}}$. Our basic building block constituting one ``layer'' in our architecture, is a type of map we dub a \emph{prismatic} map, meaning it is a lifting of the 2D mesh deformation $\planlayer$ into a 3D piecewise-linear map that operates over some plane and preserves the normal direction. Specifically, let $\p\in\rthree$ be a 3D point, and define
\begin{equation}
\liftlayer\parr{\p_x,\p_y,\p_z} \triangleq\planlayer\parr{\p_x,\p_y},\p_z, 
\end{equation}
i.e., $\liftlayer$ acts on the $xy$ coordinates of each point and preserves the $z$ coordinate. By rotating the coordinate system by a 3D rotation  $\rotation\in SO\parr{3}$ we can apply the deformation on any desired plane instead of on the main axes:

\begin{equation}
    \layer\parr{\p} \triangleq \rotation\liftlayer\parr{\rotation^T\p}.
\end{equation}
The process of mapping through $\layer$ is summarized in Algorithm~\ref{alg:point_map}. Finally, composing multiple  $\layer^i$ (defined over different planes $\rotation^i$ and with different $\planlayer^i$) yields the final 3D deformation $\map$,
\begin{algorithm}[b]
    % \SetKwInOut{Input}{Input}
    % \SetKwInOut{Output}{Output}
    Rotate point to local coordinate frame: $\q = \rotation^T\p$

    Keep only the $xy$ coordinates: $\Tilde{\q} = \parr{\q_x,\q_y}$
    
    Find triangle $\tri$ that contains $\tilde{\q}$

    
    Map through $\Psi$: $\tilde{\textbf{r}}  = A_\tri \tilde{\q} + \delta_\tri$

    Concatenate the $z$ coordinate back: $\mathbf{r} = \parr{\Tilde{\mathbf{r}}_x,\Tilde{\mathbf{r}}_y,\q_z}$

    Rotate back to global coordinates: $\layer\parr{\p} = \rotation \mathbf{r}$

    % Return the mapped point $\layer\parr{\p}$ and the triangle $\tri$
    \caption{Prismatic map  $\layer\parr{\p}$}
    \label{alg:point_map}
\end{algorithm}




\begin{equation}
\label{eq:map}
    \map = \layer^k\circ\layer^{k-1} ... \circ\layer^0.
\end{equation}
% where each $\layer^i$ is defined w.r.t a 2D piecewise-linear map $\planlayer^i$ and a rotation $\rotation^i$.

Lastly, we need to parameterize the injective 2D mesh deformation space $\planlayer: \mesh\to\rtwo$. Our reduction of the 3D injective problem to 2D sub-problems enables us to take advantage of recent advances in 2D injective mesh deformations~\cite{escher}. Originally designed for generative 2D techniques, \cite{escher} provides a parameterization of all 2D injective deformations of a given mesh, via Tutte's embedding~\cite{tutte1963draw,floater2003one,aigerman2015}. 

Following~\cite{escher}, we use the entries of the Laplacian $\lap_{ij}$ and the boundary conditions $\bdry_i$ (defined in Section~\ref{section:method:pre}) as optimizable/learnable parameters, which in turn produce the deformed vertices $\U$ of the 2D mesh, through Tutte's embedding, by solving the linear system of Eq.~\eqref{eq:tutte} w.r.t. $\lap,\bdry$.  Following the proof in~\cite{escher}, this  covers \emph{all} possible piecewise-linear maps of $\mesh$ into the convex polygon $\bdry$.  

To ensure that $\set{\bdry_i}$ form a convex polygon, we parameterize them via positive angle increments $\alpha_i>0,\sum \alpha_i=2\pi$, and define the angle $\beta_j = \sum_{i=1}^j{\alpha_i}$. $\bdry_i$ is then the intersection of the line at angle $\beta_i$ with the unit square. Hence, $\bdry$ is a function of $\alpha$.  To keep all parameters positive and bounded, we add a sigmoid and scaling function on those parameters before feeding them to the Tutte layer,
 $x'=\text{sigmoid}\parr{x}(1-2\epsilon)+\epsilon$,
 with $\epsilon=0.2$ for $\lap$ and $\epsilon=0.1$ for $\bdry$.

% To summarize, the parameters $\bdry^i,\lap^i$ define a Tutte embedding, which when calculated yields the deformed vertex positions $\U^i$. These vertex positions explicitly encode the map $\map$ and can be transmitted / stored on disk for later use, if necessary.  From $\U^i$, the 2D injective piecewise-linear map $\planlayer^i$  can be computed by Eq.~\eqref{eq:map_from_vert}. This, in turn, along with $\rotation^i$ defines $\layer^i$. 
 The parameters of a  prismatic map $\layer^i$ are thus $\theta^i=\parr{\lap^i,\bdry^i}$, and the local coordinate system $\set{\rotation^i}$. The final 3D injective piecewise-linear map $\map_\theta$ is thus parameterized by $\theta=\set{\theta^i,\rotation^i}_{i=0}^n$. We summarize the computation of $\map_\theta$ in Algorithm~\ref{alg:map_compute}. $\theta$ (and possibly $\set{\rotation^i}$) can be directly optimized with respect to an objective (Section~\ref{sec:exp:arap}), or otherwise predicted by a neural network (Section~\ref{sec:exp:learn}) -
 in both cases, we run Algorithm~\ref{alg:map_compute} at each iteration, compute the loss and back-propagate gradients back to $\theta$, as all steps in the algorithm are differentiable.
 

\vspace{-5mm}



\paragraph{Layer regularization.}
To better-condition our architecture, we can regularize its layers, ensuring each layer's Jacobian's distortion is low. We define an elastic energy measuring the Cauchy-Green strain tensor's deviation from the identity matrix $I$ at a given point $\p$ for a given map $g$, 
\begin{equation}
\label{eq:arap_energy}
    \energyarap_{g}\parr{\p} = \norm{\jac{g}{\p}^T\jac{g}{\p}-I}^2,
\end{equation}
where $\jac{g}{\p}$ is the map's Jacobian (defined in Section~\ref{section:method:pre}).
\begin{algorithm}[b]

     \caption{Computation of $\map_\theta$ from $\theta$}
    % \SetKwInOut{Input}{Input}
    % \SetKwInOut{Output}{Output}
        \label{alg:map_compute}
     \For{each deformation layer $i$}{
        Compute $\U^i$ via Tutte's embedding, by solving the linear system~\eqref{eq:tutte} defined by $\lap^i,\bdry^i$

        Compute $\planlayer^i$ from $\U^i$ using Eq.~\eqref{eq:2jac}, and store $A_\tri^i,\delta_\tri^i$ for each triangle $\tri$

        Define $\layer^i$ via $\planlayer^i$ and $\rotation^i$
    }
    Define $\map_\theta$ using all $\set{\Phi^i}_{i=0}^n$ via Eq.~\eqref{eq:map}
    
\end{algorithm}

As opposed to functional representations~\cite{realnvp,huang2020meshode}, the layer's Jacobians are enumerable (one per triangle), enabling us to compute the \emph{exact} integral of $\energyarap$  (as opposed to an approximation via sampling), by summing the energy over all Jacobians of the layer:
\begin{equation}
    \losslayer \triangleq \int_{\p\in\Omega} \energyarap_{\planlayer^i}\parr{\p} \equiv \sum_{\tri\in\T}\abs{\tri}\energyarap_{\planlayer^i}\parr{\tri},
\end{equation}
where $\abs{\tri}$ is the area of triangle $\tri$. This technique could be extended in the future to, e.g., provide absolute bounds on the distortion of each layer~\cite{kovalsky2014controlling}.

\vspace{-0.01in} %%%%%% 
\subsection{Discussion: properties of the deformation $f_\theta$}
\label{section:method:properties}

Table~\ref{tab:properties} compares different injective approaches for 3D deformations. 
% Notably, we add two properties particularly relevant to learning 3D deformations: robustness and efficient access to a full Jacobian.
Constructing $f$ through composition of mesh deformations provides it with the following desirable properties:
\\$\bullet$ \textbf{Learnable and optimizable.}
The representation of the deformation $\map_\theta$ through the unconstrained parameters $\theta$ in turn allows simple gradient-based  learning/optimization.
\\$\bullet$ \textbf{Injective, with an immediate, explicit inverse.}
 $\map$ is guaranteed to be an injective piecewise-linear map, and  we can swap the roles of $\V^i$ and $\U^i$ to immediately get the inverse  map as well as the inverse's Jacobian.
 \\$\bullet$ \textbf{Easy and fast Jacobian computation.} 
Computing the Jacobian (see supplemental) requires $2n$ multiplications of small $3\times3$ matrices, where $n$ is the number of  layers. In comparison,  methods such as RealNVP~\cite{realnvp} are designed to have efficient access to the \textit{determinant} of the Jacobian, but require $n$ multiplications of large, dense matrices to get a full Jacobian. This is even worse when second-order optimization is needed, e.g., when the Jacobians are involved in a loss (Section~\ref{sec:exp:arap}).
\\$\bullet$ \textbf{Robust and expressive.} Our framework inherits the virtues of mesh-based deformation, e.g., numerical stability, and ability to represent elaborate deformations, with this expressivity boosted by the ability to create deep compositions of these deformations.  
%Furthermore, all possible injective mesh deformations are generated from \emph{bounded} Tutte parameters, $\theta=\set{\lap,\bdry} \in\brac{-1,1}$, thus the learnable parameters of our framework are guaranteed to stay within a bounded range. 
Each Tutte layer relies on a single well behaved linear system, solved with a constant memory footprint and speed. In contrast, NeuralODE~\cite{chen2018neural} poses a hard-to-tune tradeoff between accuracy, speed, and memory consumption.
% \\$\bullet$ \textbf{Explicit geometric representation of the deformation.} \noam{weak, consider removing}The resulting deformation is explicitly represented by the list of vertices of the deformed meshes $\set{\U^i}_{i=0}^n$. This has several implications: in a learning setting (Section~\ref{sec:exp:learn}), a neural network predicts the parameters $\theta$ which define the deformation; however, this network's weights and biases are decoupled from the representation of the actual deformation. Therefore, the resolution of the deformation representation can be increased, allowing more elaborate deformations, without increasing the size of the network. On the other hand, we can increase only the network size, providing a more accurate inference, without increasing the expressivity of the deformation representation. In comparison, e.g., a functional model such as RealNVP~\cite{realnvp} predicts a  deformation via \emph{one} neural network that both serves to predict the deformation and perform inference. 
% \thibaultrmk{I liked your argument on speed as well, that an optimized map can be incorporated in NerF without requiring further network evaluations}.
%This is in contrast to other 3D injective techniques used in geometry processing~\cite{kovalsky2014controlling, campen2016bijective}, which at best lead to a non-convex constrained optimization problem that does not lend itself to, e.g., learning. 


==> bakup/4_experiments.tex <==
\vspace{-0.03in} %%%%%%
\section{Experiments}
\label{sec:exp}
We evaluate the capabilities of our injective representation both on learning a space of deformations, as well as within an optimization setting. We additionally compare to several state of the art methods for deformations - both ones that are injective as well as ones that are not. In the supplementary material, we ablate the main design choices of our method \ie number of layers, resolution of each layer, as well as the orientation of the projection planes.


\begin{figure*}[t]
\centering
\begin{overpic}[width=1\textwidth]{Figures/nerf_comparison_joint.pdf}
\put(14.5, 0){\footnotesize SPIDR~\cite{liang2022spidr}}
\put(35, 0){\footnotesize TutteNet (Ours)}
\put(59, 0){\footnotesize NeuralODE~\cite{chen2018neural}}
\put(81, 0){\footnotesize TutteNet (Ours)}
\put(8.5, 27){\footnotesize View 1}
\put(21, 27){\footnotesize NeRF-Editing~\cite{nerfediting}}
\put(39, 27){\footnotesize TutteNet (Ours)}
\put(60, 27){\footnotesize View 2}
\put(70.5, 27){\footnotesize Deforming-nerf~\cite{deformingRFCages}}
\put(87.5, 27){\footnotesize TutteNet (Ours)}
\end{overpic}
\vspace{-0.1in}

\caption{{\bf Comparing  NeRF deformation methods.} We minimize the elastic deformation energy of NeRFs under user-specified constraints (left, in green) and compare the visual quality of our results with other techniques. Non-injective methods such as NeRF-Editing~\cite{nerfediting} and Deforming-NeRF~\cite{deformingRFCages} lead to non-injective deformations due to internal inversions and intersections, in turn leading to visible artifacts.  SPIDR~\cite{liang2022spidr} relies on a hybrid SDF/point cloud representation, leading to degradation in detail (T-Rex teeth) as well non-injective artifacts (tractor). 
 We additionally compare to the only other injective method that is applicable for this experiment, NeuralODE~\cite{chen2018neural} whose injectivity avoids visual artifacts, but causes \textit{geometric} artifacts such as squashing the T-Rex's tail and the robot's eye.
}
\label{Figure:nerf_cage}
\vspace{-0.2in} %%%%% 
\end{figure*}


%%NOAM two original figs here in case we need them

% \begin{figure}[t]
% \centering
% \begin{overpic}[width=0.5\textwidth]{Figures/nerf_spidr_comparison.pdf}
% \end{overpic}
% \caption{{\bf Deforming a NeRF - comparison to point-based method.} We additionally compare with SPIDR~\cite{liang2022spidr}, a recent technique that bakes the NeRFs into a point cloud. We found that SPIDR performed better than NeRF-Editing~\cite{nerfediting} and Deforming-NeRF~\cite{deformingRFCages}, but it still suffer from local distortion due to its lack of injectivity, as shown in the inset.}
% \label{Figure:nerf_spidr}
% % \vspace{-0.2in}
% \end{figure}


% \begin{figure}[t]
% \centering
% \begin{overpic}[width=0.5\textwidth]{Figures/ode_nerf_comparison.pdf}
% \end{overpic}
% \caption{{\bf Deforming a NeRF - comparison to injective method, NeuralODE~\cite{chen2018neural}.} We compare our results to another injective NeRF deformation baseline. Both methods perform well, highlighting the importance of injectivity to avoid ray collision. \our{} produces slightly smoother deformations which better preserve texture as shown in the insets.}
% \label{Figure:nerf_ode}
% % \vspace{-0.2in}
% \noam{Bo -try fixing the locations of zoomins and also highlight squashed leg (even if you ened to use arrow)}
% \end{figure}


\subsection{Deformation of Neural Radiance Fields}
\label{sec:exp:arap}

 Neural Radiance Fields (NeRFs)~\cite{nerf} are quickly becoming one of the most popular representations for 3D scenes. Applications that use NeRFs thus require methods to manipulate and deform them, and significant research has been dedicated to NeRF deformation methods~\cite{nerfediting,NeRFshop23cage,cagenerf}. We represent a NeRF using Instant-NGP~\cite{InstantNGP},  and render it using NeRFStudio~\cite{nerfstudio}, by interfacing with their code and modifying the sampling function to go through our deformation, as we explain next.
 % All of these methods do not produce injective deformations of the entire volume, although NeRFs require sampling of ray trajectories along the deformed space, without ``collision'' of samples for correct rendering - see Figure~\ref{Figure:nerf_cage} where we compare to non-injective methods. We demonstrate the efficacy of our representation in supporting NeRF expressive deformations. 

\vspace{-0.1in} %%%%%%%%%\vspace{-3pt} 
\paragraph{Rendering the deformed NeRF.} 
 
 As discussed in previous works~\cite{deformingRFCages}, for correct rendering of a deformed NeRF, one requires both the inverse deformation as well as its Jacobian: a NeRF $N\parr{\p,\bm{r}}\rightarrow c,\sigma$ maps a point $\p$ and a view direction  $\bm{r}$ to  color $c$ and density $\sigma$, thus renderable via a ray-tracing process. Given a deformation $\map$, the point $\p$ and ray $\bm{r}$ in the deformed space correspond to the point $\p'\triangleq\map^{-1}\parr{p}$ ray $\bm{r}'\triangleq\jac{\map^{-1}}{\p}\cdot\bm{r}$ in undeformed NeRF space. Hence, we require efficient computation of $\map^{-1},\jac{\map^{-1}}{\p}$  in order to compute $N\parr{\p',\bm{r}'}$. 
 
 The only injective method, aside from ours, that supports an efficient computation of the inverse  \emph{and} its Jacobian is NeuralODE~\cite{chen2018neural,huang2020meshode,jiang2020shapeflow} - we compare to this method and show our robustness and higher accuracy. We additionally compare to non-injective methods and show the criticality of injectivity.  %Of course, as has been done in the past, non-injective methods~\cite{nerfediting,NeRFshop23cage,cagenerf} can be used, by rolling the dice and hoping they do not lead to artifacts due to lack of injectivity (see Figure~\ref{Figure:nerf_cage}).
 
 

 
 
 





 
\vspace{-3pt} 
% \vspace{-0.1in} % acknowledge  

\paragraph{Elastically deforming the NeRF.} In order to deform the NeRF, we optimize the map $\map$ to satisfy the user-specified constraints in a variational as-rigid-as-possible~\cite{arap} manner,  minimizing the elastic energy, Equation~\ref{eq:arap_energy}.  Previous methods use constructions such as proxy ``rigs'', e.g., cages~\cite{cagenerf} or point clouds~\cite{liang2022spidr}, leading to inaccuracies (e.g., when recovering the rig's geometry from an inaccurate NeRF, or when mapping between the NeRF and the rig). Our guaranteed injectivity enables deforming NeRFs directly without the tedious, brittle, proxy construction process, and we define the elastic energy of $\map_\theta$ over the density field itself:
\begin{equation}
\label{eq:lossarap}
    \lossarap = \int_{\Omega}\energyarap_{\map_\theta}\parr{\p}\sigma\parr{\p},
\end{equation}
where the integral is over  the volumetric unit cube $\Omega$,
 $\energyarap_{\map_\theta}\parr{\p}$ is defined in Equation~\eqref{eq:arap_energy}, and $\sigma$ is the NeRF's density function. The constraints are set by a user through a simple GUI,  selecting a region $\sregion$ as a ``handle'' and shifting it by a rigid motion $R$ to a new position $R\parr{\sregion}$. We enforce these constraints through an additional loss term,

\begin{equation}
    \label{eq:losshandles}
 \losshandles=\int_\sregion \norm{\map\parr{\p}-R\parr{\p}}^2.
\end{equation}
We estimate these integrals by rejection sampling on the density function $\sigma$, using a threshold of 1 on its value. Finally, we optimize the parameters $\theta$ of $\map_\theta$ w.r.t. the loss,
\begin{equation}
    \loss = \weightarap \lossarap + \weighthandles \losshandles + \weightlayer \losslayer.
\end{equation}
  We show rendered NeRFs deformed by our method in Figure~\ref{Figure:nerf_cage}, with the original NeRF shown from two views, and the selected constraints illustrated with green arrows on the left column. See more results in the supp. material.
  
% \vspace{-0.1in} % acknowledge 
\paragraph{Comparison to NeRF-deformation approaches.}  We compare our method with three state-of-the-art NeRF deformation techniques~\cite{nerfediting, liang2022spidr, deformingRFCages} in Figure~\ref{Figure:nerf_cage}. For each method, we optimize its deformation $g$ with respect to its degrees of freedom, fitting it to the injective deformation $\map$  produced by our method.  We sample points and minimize the $L^2$ distance between the images of corresponding points, $\sum_{\p}\norm{\map\parr{\p}-g\parr{p}}$, by optimizing  the deformation's degrees of freedom with respect to this loss. We perform these tests using each method's own deformation and rendering code. 

% These methods focus on speed and are more effective than us for, e.g., user-interaction. However, they are not injective, and often lead to artifacts when applied to more elaborate deformations such as the ones we show. 

 
These methods focus on interactivity and speed, often losing injectivity of 3D volumetric space when fitted to strong deformations, thus resulting in artifacts. 
 Deforming-nerf~\cite{deformingRFCages} deforms the NeRF by building a cage around it and moves points by linear dependencies with the cage's vertices. This low dimensional space cannot capture the desired deformation, and without careful attention easily leads to noninjective and tangled configurations which squash the head of the T-rex and lead to rendering artifacts that blur the texture of the robot's head. Nerf-Editing~\cite{nerfediting}'s deformation of the tail of the T-rex creates an entanglement of rendering rays with the brick floor, creating ``bleeding'' artifacts in the rendering (see zoom-in). SPIDR~\cite{liang2022spidr} bakes the NeRF into a point cloud, and we used their dataset. When deformed, it can lead to a ``discrete'' version of non-injectivity, mixing points, resulting in merged teeth for the T-Rex and incorrect rendering of the Lego model.
In contrast, our deformations remain plausible and crisp, for large displacements and for diverse shapes.

\definecolor{navyblue}{RGB}{191, 209, 229} 

\begin{table}[!t]
\centering
\small %
\setlength{\tabcolsep}{2.5pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l c c  c c | c c c} 
\hline
     \multirow{2}{*}{} & \multicolumn{2}{c}{Fitting} & \multicolumn{2}{c|}{Learning} &  \multicolumn{2}{c}{Timing (sec.)} \\ 
      & Vert. $\downarrow$ & Grad. $\downarrow$ & Vert. $\downarrow$ & Grad. $\downarrow$ & Forward  & Jacobian \\ 
     \hline
     % NICE~\cite{dinh2014nice} & - & - & - & - & \multicolumn{2}{c}{-}& -  \\ 
     RealNVP~\cite{realnvp} & 1.7 & 12.5 & 4.21 & 35.2 & \multicolumn{1}{c}{0.006}  & 136 \\ 
     i-Resnet~\cite{iresnet}  & 17.9 & 40.2  & 13.4 &  92.3 & \multicolumn{1}{c}{\cellcolor{navyblue}0.005}  & 39 \\ 
     NeuralODE~\cite{chen2018neural} &  0.19 & \cellcolor{navyblue} {2.6} &  1.24 & 25.4 &\multicolumn{1}{c}{0.11} & 0.19 \\
     \our{} (ours) & \cellcolor{navyblue} {0.15} &  4.4  & \cellcolor{navyblue}0.16 & \cellcolor{navyblue}7.7 & 0.09 & \cellcolor{navyblue}0.02 \\  
    \hline
\end{tabular}
\end{adjustbox}
\label{tab:quantitative_comp}
\caption{{\bf Quantitative comparison of injective deformation methods.} We compare the ability of our \our{}, i-ResNet~\cite{iresnet}, RealNVP~\cite{realnvp}, and NeuralODE~\cite{chen2018neural} on the human deformation fitting and learning experiments, Section~\ref{sec:exp:learn}. We report the vertex and mesh gradient terms from Equation~\ref{eqn:vertex_jacobian_loss}, both multiplied by $10^3$. 
We report average timings on the right.}
     \vspace{-0.2in}
     \label{tab:quanitative_comp}
\end{table}

\vspace*{-6pt}
% \vspace*{-0.1in}

\paragraph{Comparison to NeuralODE~\cite{chen2018neural,huang2020meshode,jiang2020shapeflow}.} As discussed above, NeuralODE is the only other method that provides both inverse and Jacobians in a computationally-feasible manner (e.g., not resorting to second-order derivation of an MLP when optimizing the Jacobian-dependent energy, Equation~\eqref{eq:lossarap}). We replaced our representation with theirs and ran the experiment with exactly the same setup. Results are shown in Figure~\ref{Figure:nerf_cage}. This comparison highlights the importance of injectivity for NeRF deformation, as neither of the two methods exhibits rendering artifacts in any scenario. However, the zoom-ins reveal geometric issues: NeuralODE  completely collapses part of the T-Rex's leg, and squashes the eye and hand of the robot, due to their proximity to one another. We additionally note that NeuralODE's numerical integration sometimes leads to running out of memory or significant stalling, when run on a large set of sample points, reducing its applicability to the NeRF rendering setting.

\subsection{Learning Injective Deformations}
\label{sec:exp:learn}
We evaluate the applicability of \our{} in a learning setting. Here, the parameters $\theta$, which define the deformation $\map_\theta$, are predicted by a neural network - note that as opposed to a standard ``hypernetwork'' which predicts parameters of another neural network, here the neural network predicts geometrically meaningful degrees of freedom and hence we do not expect significant degradation in accuracy. To quantify and evaluate our representation's ability to accurately capture injective deformations, we require a dataset with ground truths, and hence we choose to use the highly popular SMPL~\cite{smpl} model, which can generate a dataset of human meshes with groundtruth 1-to-1 correspondences between their vertices.


\begin{figure}[t]
\centering
\begin{overpic}[width=1\columnwidth]{Figures/comparison_fitting_learning.pdf}
\put(1, 17) {\rotatebox{90}{Learning}}
\put(1, 70) {\rotatebox{90}{Fitting}}
\put(10, -1) {\footnotesize Source}
\put(25, -1) {\footnotesize i-Resnet~\cite{iresnet}}
\put(42, -1) {\footnotesize NVP~\cite{realnvp}}
\put(57, -1) {\footnotesize ODE~\cite{chen2018neural}}
\put(74.5, -1) {\footnotesize Ours}
\put(89, -1) {\footnotesize GT}
\end{overpic}
\caption{{\bf Visual comparison of accuracy of injective deformation methods.} We compare the ability of our \our{}, i-ResNet~\cite{iresnet}, RealNVP~\cite{realnvp}, and NeuralODE~\cite{chen2018neural} on fitting (top) and learning (bottom) human deformations, Section~\ref{sec:exp:learn}. Our method produces highly-accurate results in the learning experiment while all others show visible artifacts. For the fitting experiment, only  NeuralODE~\cite{chen2018neural} achieves similar accuracy to ours.}

\label{Figure:fitting_comp}
\vspace{-0.2in } %%%%% 
\end{figure}

SMPL is parameterized by two sets of parameters: $P$ and $B$, dictating the human pose and body shape, resp. We generate a dataset of different body-shaped humans, each in a pair of source and target poses, $S_{B,P_s},S_{B,P_t}$. We randomly sample poses, discarding results with self-intersections. See the supp. material for full details.

Our training scheme trains the neural network to receive the source human $S_{B,P_s}$, and the target pose parameters $P_t$, and based on them predict the deformation $\map_\theta$ that deforms the source to the target $\map_\theta\parr{S_{B,P_s}}=S_{B,P_t}$. To avoid inference that relies on specific geometric structure, we encode each source human $S_{B,P_s}$ by rendering it from several viewpoints and using a visual encoder. We concatenate the output of the encoder along with the pose parameters $P_t$ into a code $\z$, which is fed into an MLP architecture that predicts the final deformation parameters $\theta$. We compute the map $\map_\theta$ via Algorithm~\ref{alg:map_compute} and use it to compute the same loss used by~\cite{aigerman2022neural} for learning mesh deformations:
{\small
\begin{equation}
\begin{aligned}
\label{eqn:vertex_jacobian_loss}
% \begin{split}
    \loss = &\norm{\map_\theta\parr{S_{B,P_s}}-S_{B,P_t}}^2+  \\
    0.1 &\norm{J\map_\theta\parr{S_{B,P_s}}-JS_{B,P_t}}^2,
% \end{split}
\end{aligned}
\end{equation}
}
where the first term is the $L_2$ distance between the deformed human mesh's vertices and the ground-truth target vertices, and the second term is the $L_2$ distance between the deformed mesh's and the ground truth mesh's intrinsic deformation gradient (note: \emph{not} the map's Jacobians), obtained by using the source mesh's gradient operator. See supplementary for full details on training. Figure~\ref{Figure:fitting_comp}, bottom shows the predicted deformations. See more results in the supp. material. 

\
% We use the meshes solely in the training phase - once the network is trained, it can directly produce volumetric injective deformations for NeRFs - We show two results in Figure~\ref{Figure:learning_nerf}, for two synthetic NeRFs created from rendered models - here the deformation transpires without any use of a mesh. 
\bo{
Since the network (trained solely on meshes) produces volumetric injective deformations, it can be readily applied to other neural fields  such as NeRFs~\cite{nerf} and SDFs~\cite{Park_2019_CVPR} -  Figure~\ref{Figure:learning_nerf} shows results of applying the same network, without retraining, on: 1) synthetic NeRF created from a rendered model; 2) real in-the-wild NeRF captured by a smartphone; 3) SDF, showing the SDF isolines as well as the marching cube reconstruction (note, though, that any deformation of an SDF violates the Eikonal equation. Hence, while the deformed field represents a valid shape, it is no longer an SDF).}
Although the network was only trained with respect to points \emph{on the surface} of the mesh, its injectivity ensures it produces meaningful deformations on the volume of the models. We additionally note that there are many methods that focus specifically on deforming NeRFs of humans (\eg SHERF~\cite{hu2023sherf}), while we use humans as a benchmark for comparing and measuring the accuracy of our method, as well as showing its generality: unlike these other techniques~\cite{chen2021animatable, neural-human-radiance-field, jiang2022selfrecon, kwon2021neural, peng2021neural, peng2023implicit, Xu2021HNeRFNR, Zhao_2022_CVPR, weng2022humannerf,su2021nerf},  we did not use any human-specific priors in the design of the representation, and the same exact method could be applied as-is to any other deformation dataset.




 \vspace{-5mm}

\paragraph{Comparison to other methods for learning injective deformations.} We use the learning experiment to compare our method with other key representatives of families of invertible neural representations: RealNVP~\cite{realnvp} (normalizing flows), i-ResNet~\cite{iresnet} (Lipschitz-bounded networks) and NeuralODE~\cite{chen2018neural} (continuous flow/ODE solutions) - all of which have been successfully applied to 3D tasks~\cite{wang2023tracking, Lei2022CaDeX, Paschalidou2021CVPR, gupta2020neural, OccupancyFlow, yang2019pointflow, jiang2020shapeflow}. We trained these methods exactly as we trained ours, with their provided code and with same number of model parameters, and performed hyperparameter sweeps to find the best-performing choices for each - refer to the supplementary. Quantitative results are shown in Table~\ref{tab:quanitative_comp}, and representative example deformations are visualized in Figure~\ref{Figure:fitting_comp}, bottom. Our method accurately learns the deformation space, achieving near-identical deformations and the lowest fitting error, while the other methods achieve higher errors, leading to visible artifacts. 
 
 As an additional experiment, we measure the ability of each technique to represent \textit{one, single deformation}, by ``overfitting'' the network (without a conditional) on a pair of source/target humans.
For this evaluation, we randomly generated 200 different-bodied humans, and sampled pose source/target pairs from the AMASS dataset~\cite{amass} for each of them. 
We show quantitative results in Table~\ref{tab:quanitative_comp} and qualitative results in Figure~\ref{Figure:fitting_comp}. 

As is evident from both experiments, RealNVP~\cite{realnvp} and i-ResNet~\cite{iresnet} produce inaccurate results compared to us, both in the learning experiment and in the fitting experiment. Indeed, they are designed to perform extremely well on high-dimensional tasks, but are less successful in 3D tasks which require very high accuracy (note the shrunk parts in Figure~\ref{Figure:fitting_comp}). RealNVP~\cite{realnvp} has low-dimensional injective coupling layers similar to us, however, each of their layers is less expressive than a Tutte layer.  i-ResNet~\cite{iresnet} achieves invertibility by regularizing ResNet blocks to have a Lipschitz constant $<1$, however, this family of functions leads to reduced expressivity to fit 3D deformations. 

While NeuralODE~\cite{chen2018neural} produces significantly less accurate deformations in the learning experiment, for the fitting experiment, they achieve results comparable to ours, with results visually close to indistinguishable in Figure~\ref{Figure:fitting_comp}, and in fact, for the fitting experiment, attain a slightly lower average error than us on the mesh-gradient fitting term (``Grad.'') while we achieve a lower vertex fitting term, see Table~\ref{tab:quanitative_comp}. The degradation in NeuralODE's performance when scaling up for the learning experiment is expected: to achieve injectivity, they leverage uniqueness of ODE solutions and plot reversible trajectories of points in 3D space - this requires numerical integration, which becomes increasingly difficult as the learned functional space represented by the neural network grows more convoluted (refer to~\cite{chen2018neural} and their discussion on their Figure 3(d)). For the fitting experiment we used the default hyperparameters from ~\cite{chen2018neural}, and for the learning experiment used the ones from~\cite{jiang2020shapeflow}.
 
 
 


% \paragraph{Fitting.}
% For the fitting task, we find that i-ResNet, RealNVP and NICE exhibit severe artifacts in fitting a single target, as shown in Figure~\ref{Figure:fitting_comp}. The deformation induced by \thibault{NICE} and and i-ResNet follow the general shape of the target but lack local geometric accuracy and squash limbs, even with large hidden layers and more layers. RealNVP achieves better overall performance but still occasionally suffers from squashed limbs as can be seen in the top row. Finally, NeuralODE and \our{} are able to accurately fit the target in all pairs we tested. This qualitative results are reflected in the quantitative evaluation we present in the left part of Table~\ref{tab:comparison}.  Our discoveries from the fitting experiment translate to the learning setting. 
% Of note, despite remarkable accuracy in the fitting experiment, NeuralODE consistantly crashes in the learning experiment because of out-of-memory issues. NeuralODE is known to be less stable than sequential neural nets because of the dynamic trade-off between speed and accuracy in the ODE solver. \thibaultrmk{Change if neccessary.}





% Based on that, we make the observation that the lack of injectivity is one of the key sources for artifacts in competing NeRF deformation approaches. It leads to ray collisions, and we hypothesis that this distorts the density and impacts the orientation at which it is observed, which leads to querying the NeRFs from viewpoints out of the training distribution. 

% Lastly, none of the SOTA baselines for NeRF deformation are well suited to learn from a dataset of human mesh deformations~\cite{amass}. This application is uniquely enabled by \our{} and we show various deformations of humanoid NeRFs in Figure~\ref{Figure:learning_nerf}.



% \noam{remove eventually}
% Nerf-Editing~\cite{nerfediting} extracts a mesh from the density function and operates by converting a surface rigid-as-possible~\cite{arap} deformation on the mesh to a volume ARAP deformation on the volume. Deforming-nerf~\cite{deformingRFCages} buids a cage around the NeRF and controls the deformation by linear dependencies between a point in the volume and the cage vertices. SPIDR~\cite{liang2022spidr} bakes the NeRF into a point cloud, then use \thibaultrmk{ask Bo} to deform the point cloud.  We note that they are other techniques to deform NeRFs, but they are also based on cages~\cite{cagenerf, NeRFshop23cage, li2023interactivecage} and on baking the radiance field~\cite{neuraleditor, neumesh}.




% \noam{put this somewhere}
% Finally, except NeuralODE which compute Jacobians via an adjoint ODE integration, none of the baselines provide quick access to optimizable Jacobians, as measured in the right side of Table~\ref{tab:quantitative_comp}. NICE and RealNVP are designed to efficiently provide the \textit{determinant} of the Jacobians. The only way to get explicit Jacobians is via higher-order differentiation which yields very slow gradient descent. For that reason, only \our{} and NeuralODE are well suited for the NeRF deformation application we discuss next. We further observe that \our{} is 3x faster than NeuralODE (80ms versus 300ms) to render deformed NeRF as both the map and the Jacobians are needed to bend the rays. 







% \begin{figure}[t]
% \centering
% \begin{overpic}[width=1\columnwidth]{Figures/comparison_fitting_learning.pdf}
% \put(1, 17) {\rotatebox{90}{Learning}}
% \put(1, 70) {\rotatebox{90}{Fitting}}
% \put(10, -0.5) {\footnotesize Source}
% \put(25, -0.5) {\footnotesize i-Resnet~\cite{iresnet}}
% \put(42, -0.5) {\footnotesize NVP~\cite{realnvp}}
% \put(57, -0.5) {\footnotesize ODE~\cite{chen2018neural}}
% \put(74.5, -0.5) {\footnotesize Ours}
% \put(89, -0.5) {\footnotesize GT}
% \end{overpic}
% \caption{{\bf Visual comparison of accuracy of injective deformation methods.} We compare the ability of our \our{}, i-ResNet~\cite{iresnet}, RealNVP~\cite{realnvp}, and NeuralODE~\cite{chen2018neural} on fitting (top) and learning (bottom) human deformations, Section~\ref{sec:exp:learn}. Our method produces highly-accurate results in the learning experiment while all others show visible artifacts. For the fitting experiment, only  NeuralODE~\cite{chen2018neural} achieves similar accuracy to ours.}

% \label{Figure:fitting_comp}
% % \vspace{-0.2in}
% \end{figure}


% \definecolor{navyblue}{RGB}{191, 209, 229} 

% \begin{table}[!t]
% \centering
% \small %
% \setlength{\tabcolsep}{2.5pt}
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{l c c  c c | c c c} 
% \hline
%      \multirow{2}{*}{} & \multicolumn{2}{c}{Fitting} & \multicolumn{2}{c|}{Learning} &  \multicolumn{2}{c}{Timing (sec.)} \\ 
%       & Vert. $\downarrow$ & Grad. $\downarrow$ & Vert. $\downarrow$ & Grad. $\downarrow$ & Forward  & Jacobian \\ 
%      \hline
%      % NICE~\cite{dinh2014nice} & - & - & - & - & \multicolumn{2}{c}{-}& -  \\ 
%      RealNVP~\cite{realnvp} & 1.7 & 12.5 & 4.21 & 35.2 & \multicolumn{1}{c}{\cellcolor{navyblue}0.006}  & 136 \\ 
%      i-Resnet~\cite{iresnet}  & 17.9 & 40.2  & 13.4 &  92.3 & \multicolumn{1}{c}{0.005}  & 39 \\ 
%      NeuralODE~\cite{huang2020meshode} &  0.19 & \cellcolor{navyblue} {2.6} &  1.24 & 25.4 &\multicolumn{1}{c}{0.11} & 0.19 \\
%      \our{} (ours) & \cellcolor{navyblue} {0.15} &  4.4  & \cellcolor{navyblue}0.16 & \cellcolor{navyblue}7.7 & 0.09 & \cellcolor{navyblue}0.02 \\  
%     \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:quantitative_comp}
% \caption{{\bf Quantitative comparison of injective deformation methods.} We compare the ability of our \our{}, i-ResNet~\cite{iresnet}, RealNVP~\cite{realnvp}, and NeuralODE~\cite{chen2018neural} on the human deformation fitting and learning experiments, Section~\ref{sec:exp:learn}. We report the vertex and mesh gradient terms from Equation~\ref{eqn:vertex_jacobian_loss}, both multiplied by $10^3$. 
% We report average timings on the right.}
%      \vspace{-0.2in}
%      \label{tab:quanitative_comp}
% \end{table}
% \begin{table}[!t]
% \centering
% \small %
% \setlength{\tabcolsep}{2.5pt}
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{l c c   | c c c} 
% \hline
%      \multirow{2}{*}{} & {Fitting} & {Learning} &  \multicolumn{3}{c}{Timing (sec.)} \\ 
%       & \multicolumn{2}{c|}{Vertex loss $ (\text{x}10^3) \downarrow$} & Forward & Map & Jacobian \\ 
%      \hline
%      % NICE~\cite{dinh2014nice} & - & - & - & - & \multicolumn{2}{c}{-}& -  \\ 
%      RealNVP~\cite{realnvp} & 1.7 &  4.21  & \multicolumn{2}{c}{\cellcolor{navyblue}0.006}  & 136 \\ 
%      i-Resnet~\cite{iresnet}  & 17.9  & 13.4  & \multicolumn{2}{c}{0.005}  & 39 \\ 
%      NeuralODE~\cite{chen2018neural} &  0.19 &  1.24  &\multicolumn{2}{c}{0.11} & 0.19 \\
%      \our{} (ours) & \cellcolor{navyblue} {0.15}   & \cellcolor{navyblue}0.16 &  0.03 & 0.06 & \cellcolor{navyblue}0.02 \\  
%     \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:quantitative_comp}
% \caption{{\bf Quantitative comparison to other classes of invertible functions.} For the task of shape fitting and deformation learning (see Sections ~\ref{sec:exp:learn} and~\ref{sec:exp:comparisons}), \our{} outperforms RealNVP~\cite{realnvp}, i-ResNet~\cite{iresnet} and performs on par with  NeuralODE~\cite{chen2018neural}.  We report the vertex error from Equation~\ref{eqn:vertex_jacobian_loss},  multiplied by $10^3$, and use 30k parameters for each method. $\dagger$ denotes runs that crashed because of OOM issues. Best performing methods are highlighted in \colorbox{navyblue}{blue}. We report timings on the right: our method computes Jacobians for the deformations 9x faster than NeuralODE, the closest competing method in terms of performance.\noam{we have to change the jacobian term here, too confusing. Let's call it something like grad. and say it's the mesh deformation gradient. Or use the }}
%      \vspace{-0.2in}
%      \label{tab:quanitative_comp}
% \end{table}


% \begin{table}[]
% \begin{subtable}[h]{0.45\textwidth}
%         \centering
%         \begin{adjustbox}{max width=0.7\textwidth}
%         \begin{tabular}{c | c c c c } 
%         \hline
%              Method & MSE ($\times 10^{-3}$) & Jacobian Error($\times 10^{-3}$) \\ 
%              \hline
%              NICE & - & - \\ 
%              RealNVP & 1.26 & 31.3 \\ 
%              i-Resnet & - & - \\ 
%              NeuralODE~\cite{huang2020meshode} & * & * \\
%              TutteNet  & 0.22 & 9.5 \\  
%             \hline
%         \end{tabular}
%         \end{adjustbox}
%         \caption{MSE and Jacobian errors for our method and RealNVP on \thibault{the test set of} the learning experiment. }
%        \label{tab:ablation:backbone}
%     \end{subtable}
%     \hfill
%     \begin{subtable}[h]{0.45\textwidth}
%         \centering
%         \begin{adjustbox}{max width=0.7\textwidth}
%         \begin{tabular}{c| c c} 
%       \hline
%             Method & MSE ($\times 10^{-4}$) & Jacobian Error($\times 10^{-3}$) \\ 
%              \hline
%              NICE & - & -\\
%              RealNVP\cite{realnvp} & 1.7 & 12.5 \\ 
%              i-Resnet\cite{iresnet} & 17.9 & 40.2 \\
%              NeuralODE\cite{huang2020meshode} & 0.19 & \textbf{2.6} \\
%              \hline
%              TutteNet  & \textbf{0.15} &  4.4 \\ 
%             \hline
%    \end{tabular}
%         \end{adjustbox}
%         \caption{MSE and Jacobian errors for our method and RealNVP on the shape fitting experiment.\thibaultrmk{make single line when complete}}
%        \label{tab:comparison}
%     \end{subtable}
%      \caption{{\bf Quantitative comparison to other classes of invertible functions.} TutteNet outperforms RealNVP~\cite{realnvp}, i-ResNet~\cite{iresnet} and performs on par with  NeuralODE~\cite{chen2018neural}.}
%      \vspace{-0.2in}
%      \label{tab:ablation2}
% \end{table}

\begin{figure}[t]
\centering
% \begin{overpic}[width=0.5\textwidth]{Figures/learning_synthetic.pdf}
\begin{overpic}[width=0.45\textwidth]{Figures/new_reposing.pdf}
\end{overpic}
\vspace{-0.05in}
\caption{\bo{ {\bf Applying the trained network to deform neural fields.} The neural network from the learning experiment (Section~\ref{sec:exp:learn}),  trained to predict deformations on a dataset of human SMPL~\cite{smpl}  meshes (top row, demonstrating the desired target pose), is seamlessly applied to deform synthetic and real \textit{NeRFs}~\cite{nerf} (middle two rows), and SDFs~\cite{Park_2019_CVPR} (bottom row). }}

% \caption{{\bf Predicting NeRF deformations.} The neural network from the learning experiment (Section~\ref{sec:exp:learn}),  trained to predict deformations on a dataset of human SMPL~\cite{smpl}  meshes (top row, demonstrating the desired target pose), is seamlessly applied to deform synthetic \textit{NeRFs}~\cite{nerf} (bottom two rows). }
\label{Figure:learning_nerf}
\vspace{-0.2in}
\end{figure}


% \subsection{Timing comparison}


\input{sec/temp_comparisons}
 







==> bakup/5_conclusion.tex <==
\section{Conclusion}
\label{conclusion}

We have presented an expressive, numerically robust, and computationally efficient representation of 3D injective deformations that can be plugged without modification into other applications requiring injective deformation modules.  

Our method has two main limitations. First, the map evaluation cannot be done at interactive times, preventing real-time rendering and interaction for the moment.
Second, deforming one part of the space may have an effect on another part, and it is non-trivial to completely localize deformations to one part of a shape. 
This is true for all the other injective deformation techniques as well.

We are excited by the possible uses of our framework, e.g., for long-range optical flow~\cite{wang2023tracking}, or to regularize non-rigid 3D registration~\cite{deng2022survey}. Additionally, use cases for other types of low-dimensional injective maps are highly attractive, e.g., for surface-to-surface mappings through common domains, which require an injective 2D map~\cite{neural_surface_maps}.
% The ability to restrict part of the domain to not deform can greatly facilitate optimization and learning and the explicit representation of the deformation via meshes could be the first step in posing geometric constraints on the deformation. 

% We see many important followups to our work. While our method is tailored for 3D deformations and is less suited than~\cite{realnvp,chen2018neural, iresnet} for deformations in higher dimensions, we believe there may be specific high-dimensional cases, where our representation's virtues will prove beneficial. Additionally, use cases for other types of low-dimensional injective maps are highly attractive, e.g., for surface-to-surface mappings through common domains, which require an injective 2D map~\cite{neural_surface_maps}. 
% \noam{check what I did here makes sense}


% Previous conclusion
% Our expressive, numerically robust, quick and explicit representation of 3D injective deformations can be plugged and used as-is, both in learning and optimization settings, without any modifications for specific tasks. 

% We are excited by the possible uses of our framework. It can be immediately used in many works that leverage injective deformations modules, e.g., for long-range optical flow work~\cite{wang2023tracking} - use of our module should lead to an immediate boost in performance \thibaultrmk{remove the claim on performance-> this is setting us up for a rebuttal experiment}.  It can be additionally used to regularize non-rigid 3D registration~\cite{deng2022survey}.

% Our method has two main limitations. First, the evaluation of the map cannot be done in interactive times, preventing, e.g., real-time rendering and interaction. An enticing option to explore is to intersect the prisms formed by the different layers, forming a compatible volumetric meshing of volumetric space before and after deformation, with 1-to-1 vertex correspondence - these meshes can be used to significantly improve the mapping process, by reducing it to a single point-in-tetrahedron computation. 
% The second limitation is that deforming one part of the space may have an effect on another part, and it's non-trivial to completely localize deformation to one part of a shape.  This is true for all injective techniques of a 3D volume. The ability to restrict part of the domain to not deform can greatly facilitate optimization and learning and the explicit representation of the deformation via meshes could be the first step in posing geometric constraints on the deformation. 

% We see many important followups to our work. While our method is tailored for 3D deformations and is less suited than~\cite{realnvp,chen2018neural, iresnet} for deformations in higher dimensions, we believe there may be specific high-dimensional cases, where our representation's virtues will prove beneficial. Additionally, use cases for other types of low-dimensional injective maps are highly attractive, e.g., for surface-to-surface mappings through common domains, which require an injective 2D map~\cite{neural_surface_maps}. 
% \noam{check what I did here makes sense}

% {\scriptsize \noindent \textbf{Acknowledgments} We would like to acknowledge  support from NSF IIS-2047677,
% HDR-1934932, CCF-2019844, and IARPA WRIVA program.}

==> bakup/7_rebuttal.tex <==
\textbf{Dear reviewers}, thank you for your time and effort -  we are happy that all appreciate our paper!

\noindent \textbf{\revB: Code release?}
We will release the code.

\noindent \textbf{\revA: Is injectivity guaranteed?}  \textit{It is mathematically guaranteed that the predicted deformation will be injective}. 
Our method doesn’t slice the volume, but rather each layer injectively deforms 3D space over a different deformation \textit{plane} (see Eq. 4 in main paper).

\noindent \textbf{\revA: Rotation Matrix $R$?}
$R$ is the coordinate system for  the deformation plane (Eq. 5) and a parameter of the layers.  
We show 2 possible plane policies  (Table 2, supp.): alternating planes over the 3 main axes; and letting a network predict the planes. It is not trained from a user choice rather learned in an unsupervised manner (L261-263). 

\noindent \textbf{\revA: The network is tailored to SMPL?}
\textit{No}. We use the exact same structure in all experiments (L541), only modifying number of layers and mesh resolution. Our method is not tailored to SMPL specifically in any way, and given any other dataset could be applied without any modifications.   

\noindent \textbf{\revC: Deforming SDFs and Gaussian Splats?} Our method can deform SDFs as-is, with the same exact technique as for NeRFs. The inset shows an SDF deformed using our network, and meshed via marching cubes. \begin{wrapfigure}[6]{r}{1.8cm}
\vspace{-15pt}
\hspace{-22pt}
\includegraphics[width=2.5cm]{Figures/sdf.pdf}
% \caption{Surface reconstruction from SDF deformation. }\label{wrap-fig:1}
\end{wrapfigure}  We will add an experiment showing deformation of other SDFs. Note, that any deformation of an SDF does violate the Eikonal equation. Regarding Gaussian Splats: they provide remarkable novel-view synthesis, but do not well-represent the underlying geometry, hence visuals break under deformation  (confirmed by the authors of that paper). 

\noindent \textbf{\revA: Isometric regularization restricts to isometric deformation?} Eq. 7 encourages  each \textit{layer} to be regularized, similarly to weight-regularization of a neural network. Even if each layer has very low isometric distortion (e.g., $1.5$), the layers' composition can still represent very high distortion (10 layers could have distortion of $1.5^{10}\approx57$)), if needed.





% \noindent \textbf{Layer Regularization}
% The layer regularization is like the weight regularization in CNN. Our model is suitable for most types of deformations because each layer has a small deformation and they can be composed to large deformation in the end. 



\noindent \textbf{\revB:  NeRF deformation baselines have only small artifacts.} Fig. 3: Deforming-Nerf on the T-Rex shows noticeable issues, and the small holes in the Lego for Nerf-Editing are also disturbing and immediate to notice in a video, as they flicker and change as the viewpoint is changing. 

\noindent \textbf{\revB: Quantitative comparison on synthetic data.}
Our core contribution is not directly NeRF-focused, but rather a generic method for learning injective 3D deformations. Thus Table 2  quantitatively compares to previous injective techniques on {synthetic} data, as it is the only data with geometric GT. We show qualitative examples of NeRF deformation as a main application, however unfortunately, there's no dataset with GT for quantitative evaluation of novel-view synthesis editing.  

\noindent \textbf{\revB: More Qualitative Results on real-captured Data.}
We will add more qualitative results on real NeRFs we captured with a smartphone, such as these ones:
% \ref{Figure:real_nerf}. 


\begin{figure}[h]
\centering
\vspace{-0.1in}
\begin{overpic}[width=0.45\textwidth]{Figures/real_nerf_v3.pdf}
\end{overpic}
\vspace{-0.15in}
% \caption{More qualitative results on real NeRF. }
% \label{Figure:real_nerf}
% \vspace{-0.2in}
\end{figure}

% \begin{figure}[t]
% \centering
% \begin{overpic}[width=0.45\textwidth]{Figures/real_nerf.pdf}
% \end{overpic}
% \vspace{-0.1in}
% \caption{More qualitative results on real NeRF. }
% \label{Figure:real_nerf}
% \vspace{-0.2in}
% \end{figure}

\noindent \textbf{\revB: Non-local/highly non-isometric deformation.} These possible concerns apply to \emph{any} injetive method. Empirically, our experiments show our method can learn isometric priors as well as localize deformations to, e.g., different limbs of humans (Fig. 4). We haven't observed deterioration in higher resolutions (e.g., Table 1 in supp.). 





\noindent \textbf{\revB: Boundary deformation?}
We learn deformations of the  cube $[-1, 1]^3$, but objects are normalized to $[-0.7, 0.7]^3$,  hence their boundary is within the cube and is deformed freely.




\noindent \textbf{\revC: Deformation through mesh presupposes the object is a surface?}
We focus on learning injective \textit{volumetric} deformations and not of surfaces. The 2D mesh is not of the surface, but a proxy used to define a volumetric deformation in each layer (see L216-218 and teaser).

% We deform the entire 3D space with 2D mesh deformation. The input shapes are just volumetric points. The process is: (1). triangulate and deform the space, (2). deform points based on barycentric interpolation to the space mesh vertices. 
% The objects are not surface-like. In the NeRF deformation, we directly take the volumetric points with large density predictions and apply deformations on them. 


\noindent \textbf{\revC: Reduction from 3D to 2D leads to error?}
% \bo{Noam needs to think} 
As a finite representation TutteNet is of course limited to a (piecewise-linear) subset of the huge space of injective deformations. Proving a \textit{universal approximation theorem} for injective deformations is unexplored territory as far as we know, and we mark it as interesting future work.

% \begin{wrapfigure}{r}{3cm}
% \includegraphics[width=3cm]{Figures/sdf.pdf}
% \caption{Surface reconstruction from SDF deformation. }\label{wrap-fig:1}
% \end{wrapfigure} 

\noindent \textbf{\revC: Inferring deformation requires additional computation.}
Our timings (Table 2 in the main paper) are on par with alternative injective techniques.
Note, a significant part of computation is spent solving relatively-small sparse linear systems, and we used an off-the-shelf generic solver. Integrating tailor-made solvers could release this bottleneck.

\noindent \textbf{\revB: Laplacian?}
We treat the entries of the laplacian as part of the learnable parameters $\theta$ (see Fig. 2 and L238-240), which control the deformation while ensuring injectivity, hence it is not a fixed cotan laplacian or such.

\noindent \textbf{\revA: Number of Layers and mesh resolution?}
These are similar to depth/width in, e.g., MLPs. They are chosen based on a trade-off between accuracy and computation time (see Table 1 and Figure 4 in the supmat). 
 
\noindent \textbf{\revA: Choice of $\epsilon$?}
We require values in the range $(0,1)$, hence operate in the range $[\epsilon, 1-\epsilon]$ - from our tests, the exact choice of a small  $\epsilon$ is not critical.





% \noindent \textbf{\revD: Future research}. Thank you for the pointer!

\noindent \textbf{\revA: Kinematic Constraints?}
Without running empirical trials on such a dataset, it is impossible to guarantee performance. However, our method is generic, and would be applicable to learn kinematic constraints.

\noindent \textbf{\revD:  Is $\beta_j$ scaled  by $2\pi / \sum \alpha_i$?} Exactly!  We will clarify the text.



==> sec/7_rebuttal.tex <==
\textbf{Dear reviewers}, thank you for your time and effort -  we are happy that all appreciate our paper!

\noindent \textbf{\revB: Code release?}
We will release the code.

\noindent \textbf{\revA: Is injectivity guaranteed?}  \textit{It is mathematically guaranteed that the predicted deformation will be injective}. 
Our method doesn’t slice the volume, but rather each layer injectively deforms 3D space over a different deformation \textit{plane} (see Eq. 4 in main paper).

\noindent \textbf{\revA: Rotation Matrix $R$?}
$R$ is the coordinate system for  the deformation plane (Eq. 5) and a parameter of the layers.  
We show 2 possible plane policies  (Table 2, supp.): alternating planes over the 3 main axes; and letting a network predict the planes. It is not trained from a user choice rather learned in an unsupervised manner (L261-263). 

\noindent \textbf{\revA: The network is tailored to SMPL?}
\textit{No}. We use the exact same structure in all experiments (L541), only modifying number of layers and mesh resolution. Our method is not tailored to SMPL specifically in any way, and given any other dataset could be applied without any modifications.   

\noindent \textbf{\revC: Deforming SDFs and Gaussian Splats?} Our method can deform SDFs as-is, with the same exact technique as for NeRFs. The inset shows an SDF deformed using our network, and meshed via marching cubes. \begin{wrapfigure}[6]{r}{1.8cm}
\vspace{-15pt}
\hspace{-22pt}
\includegraphics[width=2.5cm]{Figures/sdf.pdf}
% \caption{Surface reconstruction from SDF deformation. }\label{wrap-fig:1}
\end{wrapfigure}  We will add an experiment showing deformation of other SDFs. Note, that any deformation of an SDF does violate the Eikonal equation. Regarding Gaussian Splats: they provide remarkable novel-view synthesis, but do not well-represent the underlying geometry, hence visuals break under deformation  (confirmed by the authors of that paper). 

\noindent \textbf{\revA: Isometric regularization restricts to isometric deformation?} Eq. 7 encourages  each \textit{layer} to be regularized, similarly to weight-regularization of a neural network. Even if each layer has very low isometric distortion (e.g., $1.5$), the layers' composition can still represent very high distortion (10 layers could have distortion of $1.5^{10}\approx57$)), if needed.





% \noindent \textbf{Layer Regularization}
% The layer regularization is like the weight regularization in CNN. Our model is suitable for most types of deformations because each layer has a small deformation and they can be composed to large deformation in the end. 



\noindent \textbf{\revB:  NeRF deformation baselines have only small artifacts.} Fig. 3: Deforming-Nerf on the T-Rex shows noticeable issues, and the small holes in the Lego for Nerf-Editing are also disturbing and immediate to notice in a video, as they flicker and change as the viewpoint is changing. 

\noindent \textbf{\revB: Quantitative comparison on synthetic data.}
Our core contribution is not directly NeRF-focused, but rather a generic method for learning injective 3D deformations. Thus Table 2  quantitatively compares to previous injective techniques on {synthetic} data, as it is the only data with geometric GT. We show qualitative examples of NeRF deformation as a main application, however unfortunately, there's no dataset with GT for quantitative evaluation of novel-view synthesis editing.  

\noindent \textbf{\revB: More Qualitative Results on real-captured Data.}
We will add more qualitative results on real NeRFs we captured with a smartphone, such as these ones:
% \ref{Figure:real_nerf}. 


\begin{figure}[h]
\centering
\vspace{-0.1in}
\begin{overpic}[width=0.45\textwidth]{Figures/real_nerf_v3.pdf}
\end{overpic}
\vspace{-0.15in}
% \caption{More qualitative results on real NeRF. }
% \label{Figure:real_nerf}
% \vspace{-0.2in}
\end{figure}

% \begin{figure}[t]
% \centering
% \begin{overpic}[width=0.45\textwidth]{Figures/real_nerf.pdf}
% \end{overpic}
% \vspace{-0.1in}
% \caption{More qualitative results on real NeRF. }
% \label{Figure:real_nerf}
% \vspace{-0.2in}
% \end{figure}

\noindent \textbf{\revB: Non-local/highly non-isometric deformation.} These possible concerns apply to \emph{any} injetive method. Empirically, our experiments show our method can learn isometric priors as well as localize deformations to, e.g., different limbs of humans (Fig. 4). We haven't observed deterioration in higher resolutions (e.g., Table 1 in supp.). 





\noindent \textbf{\revB: Boundary deformation?}
We learn deformations of the  cube $[-1, 1]^3$, but objects are normalized to $[-0.7, 0.7]^3$,  hence their boundary is within the cube and is deformed freely.




\noindent \textbf{\revC: Deformation through mesh presupposes the object is a surface?}
We focus on learning injective \textit{volumetric} deformations and not of surfaces. The 2D mesh is not of the surface, but a proxy used to define a volumetric deformation in each layer (see L216-218 and teaser).

% We deform the entire 3D space with 2D mesh deformation. The input shapes are just volumetric points. The process is: (1). triangulate and deform the space, (2). deform points based on barycentric interpolation to the space mesh vertices. 
% The objects are not surface-like. In the NeRF deformation, we directly take the volumetric points with large density predictions and apply deformations on them. 


\noindent \textbf{\revC: Reduction from 3D to 2D leads to error?}
% \bo{Noam needs to think} 
As a finite representation TutteNet is of course limited to a (piecewise-linear) subset of the huge space of injective deformations. Proving a \textit{universal approximation theorem} for injective deformations is unexplored territory as far as we know, and we mark it as interesting future work.

% \begin{wrapfigure}{r}{3cm}
% \includegraphics[width=3cm]{Figures/sdf.pdf}
% \caption{Surface reconstruction from SDF deformation. }\label{wrap-fig:1}
% \end{wrapfigure} 

\noindent \textbf{\revC: Inferring deformation requires additional computation.}
Our timings (Table 2 in the main paper) are on par with alternative injective techniques.
Note, a significant part of computation is spent solving relatively-small sparse linear systems, and we used an off-the-shelf generic solver. Integrating tailor-made solvers could release this bottleneck.

\noindent \textbf{\revB: Laplacian?}
We treat the entries of the laplacian as part of the learnable parameters $\theta$ (see Fig. 2 and L238-240), which control the deformation while ensuring injectivity, hence it is not a fixed cotan laplacian or such.

\noindent \textbf{\revA: Number of Layers and mesh resolution?}
These are similar to depth/width in, e.g., MLPs. They are chosen based on a trade-off between accuracy and computation time (see Table 1 and Figure 4 in the supmat). 
 
\noindent \textbf{\revA: Choice of $\epsilon$?}
We require values in the range $(0,1)$, hence operate in the range $[\epsilon, 1-\epsilon]$ - from our tests, the exact choice of a small  $\epsilon$ is not critical.





% \noindent \textbf{\revD: Future research}. Thank you for the pointer!

\noindent \textbf{\revA: Kinematic Constraints?}
Without running empirical trials on such a dataset, it is impossible to guarantee performance. However, our method is generic, and would be applicable to learn kinematic constraints.

\noindent \textbf{\revD:  Is $\beta_j$ scaled  by $2\pi / \sum \alpha_i$?} Exactly!  We will clarify the text.


